Approximate streamsurfaces for flow visualization

Instantaneous features of three-dimensional velocity fields are most directly visualized via streamsurfaces. It is generally unclear, however, which streamsurfaces one should pick for this purpose, given that infinitely many such surfaces pass through each point of the flow domain. Exceptions to this rule are vector fields with a nondegenerate first integral whose level surfaces globally define a continuous, one-parameter family of streamsurfaces. While generic vector fields have no first integrals, their vortical regions may admit local first integrals over a discrete set of streamtubes, as Hamiltonian systems are known to do over Cantor sets of invariant tori. Here we introduce a method to construct such first integrals approximately from velocity data, and show that their level sets indeed frame vortical features of the velocity field in examples in which those features are known from Lagrangian analysis. Moreover, we test our method in numerical data sets, including a flow inside a V-junction and a turbulent channel flow. For the latter, we propound an algorithm to pin down the most salient barriers to momentum transport up to a given scale providing a way out of the occlusion conundrum that typically accompanies other vortex visualization methods.

==> config.tex <==
% -----------------------------------------------------------------------------
% Section headings format
% -----------------------------------------------------------------------------
%\titleformat{\section}{\bfseries}{\thesection}{14pt}{\linespread{1.0}}
%\titleformat{\subsection}{\bfseries}{\thesubsection}{12pt}{\linespread{1.0}}

%\titleformat{\chapter}{\large\bfseries}{\thesection}{1em}{\linespread{1.0}\large}

%\titleformat{\chapter}[display]
%   {\bfseries\filright}
%   {ΚΕΦΑΛΑΙΟ\space\thechapter}
%   {16pt}
%   {\linespread{1.0}}

% -----------------------------------------------------------------------------
% MARGINS
% -----------------------------------------------------------------------------
    \newlength \pageheight
    \newlength \pagewidth
    \pageheight     297mm
    \pagewidth      210mm
    \textheight     225mm
    \topmargin      0.2in    % up-down position here 0.80:HP4ML, 0.13:HP720C
    \headheight     5mm
    \headsep        5mm
    \textwidth      150mm
    \oddsidemargin  4.0mm    % odd margin  (monos) (+ 1in)
    \evensidemargin 4.0mm    % even margin (zygos) (+ 1in)

%\renewcommand{\baselinestretch}{1.15}

% -----------------------------------------------------------------------------
% LOOSEN FLOATING PARAMETERS
% -----------------------------------------------------------------------------
\renewcommand{\topfraction}{.85}
\renewcommand{\bottomfraction}{.7}
\renewcommand{\textfraction}{.15}
\renewcommand{\floatpagefraction}{.66}
\renewcommand{\dbltopfraction}{.66}
\renewcommand{\dblfloatpagefraction}{.66}
\setcounter{topnumber}{9}
\setcounter{bottomnumber}{9}
\setcounter{totalnumber}{20}
\setcounter{dbltopnumber}{9}

% -----------------------------------------------------------------------------
% headers
% -----------------------------------------------------------------------------
%\pagestyle{fancy}

%\renewcommand{\footrulewidth}{0.3pt}
%\newcommand{\san}{\small}
%\fancyhf{}
%\fancyhead[LE,RO]{\bf \thepage}
%\fancyhead[LO]{\san \rightmark}
%\fancyhead[RE]{\san \leftmark}

\pagestyle{fancy}
%\renewcommand{\sectionmark}[1]{\markright{\thesection.\ #1}}


%\renewcommand{\chaptermark}[1]{\markboth{#1}{}}
%\newcommand{\san}{\small}
%\fancypagestyle{style1}{
%\fancyhf{}
%\fancyhead[RE]{\nouppercase\thechapter.~\leftmark}
%\fancyhead[RE]{\thechapter.~\leftmark}
%\fancyhead[RE]{\nouppercase \leftmark}
%\fancyhead[LO]{\nouppercase \rightmark}
%\fancyhead[LE,RO]{\thepage}
%\renewcommand{\footrulewidth}{0.4pt}
%\renewcommand{\headrulewidth}{0.4pt}
%\fancyhead[LO]{\textgreek{\san \nouppercase \rightmark}}
%\fancyhead[RE]{\textgreek{\san \nouppercase \leftmark}}
%\fancyfoot[L]{\bf \thepage}


%\fancypagestyle{style2}{
%	\fancyhf{}
%	\fancyhead[RE]{\nouppercase}
%	%\fancyhead[RE]{\thechapter.~\leftmark}
%	%\fancyhead[RE]{\nouppercase \leftmark}
%	\fancyhead[LO]{\nouppercase \rightmark}
%	\fancyhead[LE,RO]{\bf \thepage}}
%	%\fancyhead[LO]{\textgreek{\san \nouppercase \rightmark}}
%	%\fancyhead[RE]{\textgreek{\san \nouppercase \leftmark}}
%	%\fancyfoot[L]{\bf \thepage}

%\pagestyle{style1}

% -----------------------------------------------------------------------------
% HYPERREFS
% -----------------------------------------------------------------------------
%\hypersetup{
%pdfstartview={FitH},
%breaklinks={true},
%pdfpagemode={UseOutlines},
%colorlinks,
%linkcolor={blue},
%citecolor={red},
%urlcolor={cyan},
%}

% -----------------------------------------------------------------------------
% HYPHENATION
% -----------------------------------------------------------------------------
%\righthyphenmin=1
%\lefthyphenmin=1
%\tolerance=1
%\emergencystretch=\maxdimen
%\hyphenpenalty=10000
%\hbadness=10000

% -----------------------------------------------------------------------------
% ACKNOWLEDGEMENTS
% -----------------------------------------------------------------------------
\newcommand\acknowledge{
\@startsection{paragraph}%name
{100}%level
{0pt}%indent
{\baselineskip}%beforeskip
{0.5\baselineskip}%afterskip
{\bfseries}%style
}

%\setlength{\abovedisplayskip}{0pt}
%\setlength{\belowdisplayskip}{0pt}
%\setlength{\abovedisplayshortskip}{0pt}
%\setlength{\belowdisplayshortskip}{0pt}

% -----------------------------------------------------------------------------
% Macros
% -----------------------------------------------------------------------------
\input{macros}
\def\ten#1{\overline{\overline #1}}
\def\MSE{\emph{MSE}}
\def\til#1{\overline #1}
%\input{macrosxef}
%\input{macrosdim}
%\input{macroskirk}
\input{macrosdummy}

\MakeRobust{\overrightarrow}

\setcounter{secnumdepth}{3}

\newcommand{\ENG}[1]{ \emph{ \textbf{\eng{#1}} } }

% -----------------------------------------------------------------------------
% line spacing
% -----------------------------------------------------------------------------
\spacing{1.0}

% -----------------------------------------------------------------------------
% graphics
% -----------------------------------------------------------------------------
\graphicspath{{./figs/}}
\DeclareGraphicsExtensions{.eps,.ps,.jpg}

\renewcommand{\baselinestretch}{1.2}


==> least_squares.tex <==
%\chapter{\texttt{BarrierTool} Manual}

\section{Ordinary least squares and ridge regression}
\label{app:least_squares}

\begin{theorem}
	Let $\mathbf{C}=\mathbf{U}\mathbf{\Sigma} \mathbf{V}^{*}$ be the singular value decomposition of a matrix $\mathbf{C}$. The minimum-norm solution to
	\begin{equation}
	\min_{\mathbf{x}} ||\mathbf{C} \mathbf{x} - \mathbf{b}||
	\end{equation}
	is given as
	\begin{equation}
	\hat{\mathbf{x}} = \mathbf{V} \mathbf{\Sigma}^{+} \mathbf{U}^{*} \mathbf{b}
	\end{equation}
	where
	\begin{equation}
	\mathbf{\Sigma}^{+} = \left( \mathbf{\Sigma}_r^{+} \mkern7mu 0\right) \in \mathbb{C}^{n \times m}, \quad \mathbf{\Sigma}_r^{+}  = \mathrm{diag} \left(  \frac{1}{\sigma_1}, \dotsc, \frac{1}{\sigma_r}, 0, \dotsc, 0 \right) \in \mathbb{C}^{n \times n}
	\end{equation}
\end{theorem}
\begin{proof}
We want to find the minimal $||\mathbf{x}||$ that simultaneously minimizes $|| \mathbf{C} \mathbf{x} - \mathbf{b}||$. This can be written as $|| \mathbf{U}\mathbf{\Sigma} \mathbf{V}^{*} \mathbf{x} - \mathbf{b} ||$, or
$|| \mathbf{U}(\mathbf{\Sigma} \mathbf{V}^{*} \mathbf{x} - \mathbf{U}^{*}\mathbf{b}) ||$, or
$|| \mathbf{\Sigma} \mathbf{V}^{*} \mathbf{x} - \mathbf{U}^{*}\mathbf{b} ||$ because $\mathbf{U}$ is a unitary matrix and does not alter the norm of the vectors it acts on. Using $\mathbf{y} = \mathbf{V}^{*} \mathbf{x}$ and $\mathbf{c} = \mathbf{U}^{*} \mathbf{b}$, we want to minimize $|| \mathbf{\Sigma} \mathbf{y} - \mathbf{c} ||$. Upon expanding this we have
\begin{equation}
\left[\begin{array}{cccccc}
\sigma_{1} & 0 &  &  &  & 0\\
0 & \ddots &  &  &  & 0\\
&  & \sigma_{r}\\
\vdots &  &  & 0 &  & \vdots\\
&  &  &  & \ddots\\
0 &  & \ldots &  &  & 0
\end{array}\right]\left[\begin{array}{c}
y_{1}\\
\vdots\\
y_{r}\\
y_{r+1}\\
\vdots\\
y_{n}
\end{array}\right]-\left[\begin{array}{c}
c_{1}\\
\vdots\\
c_{r}\\
c_{r+1}\\
\vdots\\
c_{n}
\end{array}\right]
\end{equation}
From this, we obtain explicitly $y_i = \frac{c_i}{\sigma_i}$ for $i = 1,\dotsc,r$, whereas we set $y_i = 0$ for $i = r+1, \dotsc, n$ because we want the minimum-norm solution for $\mathbf{x}$ or, equivalently $\mathbf{y}$, since these two vectors are connected through a unitary transformation. We therefore have $\mathbf{y} = \mathbf{\Sigma}^{+} \mathbf{c}$ or upon substitution $\hat{\mathbf{x}} = \mathbf{V} \mathbf{\Sigma}^{+} \mathbf{U}^{*} \mathbf{b}$. We note that uniqueness here stems from the unit-norm requirement.
\end{proof}

\iffalse

In the case of ridge regression we seek to minimize the quantity $|| \mathbf{C} \mathbf{x} - \mathbf{b}||^2 + || \mathbf{x}||^2$ instead. Following a similar approach as above the solution is given as
\begin{equation}
\hat{\mathbf{x}}_{ridge} = \mathbf{V} \left( \mathbf{\Sigma}^{\top} \mathbf{\Sigma} + \lambda \mathbf{I}\right)^{-1} \mathbf{\Sigma}^{\top} \mathbf{U}^{*} \mathbf{b}
\end{equation}

\fi

==> macros.tex <==
\newcommand{\eng}[1]{\textlatin{#1}}    %Quick english... 
\newcommand{\mbf}[1]{\mathbf{#1}}       %This is bold in math mode 
\newcommand{\ol}[1]{\overline{#1}} 
\newcommand{\pp}{\partial}              %partial is too big! 
\newcommand{\mvec}[1]{\boldsymbol{#1}}      %vector definition
\newcommand{\mvun}[1]{\widehat{\mvec{#1}}}%unit vector
\newcommand{\un}[1]{\widehat{#1}}        %unit something
\newcommand{\nodim}[1]{\breve{#1}}      %non-dimensinal definition
\newcommand{\jac}[1]{\underline{#1}}    %Jacobian
\newcommand{\roe}[1]{\widetilde{#1}}    %Roe symbol
\newcommand{\rjac}[1]{\roe{\jac{#1}}}   %Roe Jacobian
\newcommand{\rvec}[1]{\roe{\mvec{#1}}}   %Roe Vector

\newcommand{\iintsub}[1]{\underset{#1}{\iint}}
\newcommand{\intsub}[1]{\underset{#1}{\int}}
\newcommand{\ubs}[2]{\underset{#1}{\underbrace{#2}}}
 
\newcommand{\mysize}{0.4\textwidth}



==> macrosdummy.tex <==
\newcommand{\p}{\partial}
\newcommand{\arr}{\overrightarrow}


==> packages.tex <==
%-----------------------   P A C K A G E S   ---------------------------%
\usepackage{multicol}
\usepackage{xspace}
\usepackage[unicode,linktocpage,breaklinks]{hyperref}
\usepackage{textcomp}
\usepackage{breakurl}


% >> Math package:
\usepackage{amsmath}
\usepackage{amsthm}
\usepackage{amsbsy}
\usepackage{amstext}
\usepackage{amssymb}
\usepackage{amsfonts}
\usepackage{nicefrac}
\usepackage{mathtools}


\usepackage[greek,english]{babel}
\usepackage[utf8x]{inputenc}
%\usepackage[iso-8859-7]{inputenc}
%\usepackage{kerkis}
\usepackage{parskip}

% improved layout of figure captions with extra margin, smaller font than text
\usepackage[margin=10pt,font=small,labelfont=bf]{caption}
%\usepackage{xltxtra}

\usepackage{graphicx}
\usepackage{epstopdf}
\usepackage{latexsym}
\usepackage{babel,varioref}
\usepackage{setspace}
%\usepackage{subfigure}
\usepackage{fixltx2e}
\usepackage{pstricks}
\usepackage{latexsym} 
\usepackage{multirow}
\usepackage{array}
\usepackage{color}
\usepackage{algorithm}
%\usepackage[]{algorithm2e}
\usepackage{algorithmicx}
\usepackage{algpseudocode}
\usepackage{listings}
\usepackage{enumerate}
\usepackage{mwe}
%\usepackage{subfig}
\usepackage{subcaption}
\usepackage{verbatim}
\usepackage{bm}
\usepackage{wrapfig}


\makeatletter
\AtBeginDocument{%
	\expandafter\def\expandafter\originalTeX\expandafter{%
		\expandafter\@tempcnta\number253\expandafter\relax\originalTeX}%
}
\makeatother

\usepackage{babelbib}
\usepackage{url}
% \usepackage{multibib}

\usepackage{caption}

% TABLE OF CONTENTS PACKAGES
\usepackage[subfigure]{tocloft}
\usepackage[nottoc]{tocbibind}

% Line Spacing
\usepackage{setspace}
%\usepackage[nodisplayskipstretch]{setspace}

% fancy header
\usepackage{fancyhdr} 
%\usepackage[unicode]{hyperref}

% footnotes: waring in case of splitted footnote
\usepackage{fnbreak}

% extra controlabity for enumerators
\usepackage{enumitem}

% Section headings format
\usepackage{titlesec}
%\usepackage{sectsty}

% abstract
%\newenvironment{abstract}{}{}
%\usepackage{abstract}

% appendix
\usepackage{appendix}

\usepackage{lipsum}

% links
\usepackage{hyperref}
\hypersetup{
	colorlinks,
	citecolor=blue,
	filecolor=blue,
	linkcolor=black,
	urlcolor=cyan
}
